DialogCC: An Automated Pipeline for Creating High-Quality Multi-Modal Dialogue Dataset

As sharing images in an instant message is a crucial factor, there has been active research on learning an image-text multi-modal dialogue models. However, training a well-generalized multi-modal dialogue model remains challenging due to the low quality and limited diversity of images per dialogue in existing multi-modal dialogue datasets. In this paper, we propose an automated pipeline to construct a multi-modal dialogue dataset, ensuring both dialogue quality and image diversity without requiring minimum human effort. In our pipeline, to guarantee the coherence between images and dialogue, we prompt GPT-4 to infer potential image-sharing moments - specifically, the utterance, speaker, rationale, and image description. Furthermore, we leverage CLIP similarity to maintain consistency between aligned multiple images to the utterance. Through this pipeline, we introduce DialogCC, a high-quality and diverse multi-modal dialogue dataset that surpasses existing datasets in terms of quality and diversity in human evaluation. Our comprehensive experiments highlight that when multi-modal dialogue models are trained using our dataset, their generalization performance on unseen dialogue datasets is significantly enhanced. We make our source code and dataset publicly available.

==> sections/supp_sections/dicussion.tex <==
\section{Discussion} \label{supp_sec:discussion}

\paragraph{Dicussion about Societal Impact.}
As mentioned in the Limitation section, we need to carefully consider potential gender-bias issues for the fairness multi-modal dialogue search model. To mitigate this potential issue, we think of three strategies to remove the potential gender bias problem. 
First, we can adopt a fair sampling approach~\cite{wang2021gender} during training via contrastive learning, which considers gender distribution to be fair. 
Second, we can adopt post-hoc methods, such as Post-hoc Bias Mitigation (PBM)~\cite{kong2024mitigating} or Post-processing debiasing~\cite{wang2021gender}, in the dataset construction phase, particularly during alignment with CLIP. 
Lastly, we alternatively leverage fairness-focused vision-and-language pre-trained models, such as FairCLIP~\cite{wang2022fairclip}, as a function $f(\cdot)$. These strategies aim to minimize gender bias as effectively as possible.

Instead of generating social dialogues with GPT-4, we use verified dialogue datasets (\ie EmpatheticDialogues, Wizard-of-Wikipedia, DailyDialog, BlendedSkillTalk, PersonaChat) as seed dialogue to identify potential image-sharing moments in these seed dialogues. Therefore, we did not conduct a direct safety filtering process for the social dialogue datasets. However, since LLMs can generate harmful content, we can use tools like the Rewire API to remove potentially toxic content during the process of creating image descriptions with GPT-4. Additionally, GPT-4 could produce biased results due to name bias in the given dialogues~\cite{sheng2021revealing}, we randomly replaced all names in conversations with Top-10K names of US SSN applicants from 1990 to 2021. Following the previous studies~\cite{smith2021hi,kim2022soda}, this approach ensures a broad representation of names from diverse genders and ethnic backgrounds.

==> tables/main_tables/image_aug_results.tex <==
{\renewcommand{\arraystretch}{1.35}
\begin{table}[t]
\centering
\begin{adjustbox}{width=0.6\columnwidth}
\begin{tabular}{lcccc}
\toprule
         & \multicolumn{2}{c}{MMDD} & \multicolumn{2}{c}{DialogCC} \\ \cmidrule{2-5}
Aug $\downarrow$      & R@1        & $\Delta$      & R@1          & $\Delta$        \\ \midrule
Baseline & 13.09      & -           & 8.35         & -             \\ \midrule
cutout   & 13.62      & -0.54       & 7.68         & 0.67          \\
dropout  & 10.65      & 2.44        & 7.66         & 0.69          \\
zoom-in  & 11.48      & 1.61        & 7.33         & 1.02          \\
zoom-out & 11.43      & 1.66        & 7.73         & 0.62          \\
rotation & 12.89      & 0.20        & 7.71         & 0.65          \\
shearing & 12.35      & 0.73        & 7.49         & 0.86          \\
noise    & 10.60      & 2.49        & 7.74         & 0.61          \\
blur     & 12.94      & 0.15        & 7.92         & 0.44          \\ \midrule
Avg.     & 11.99      & 1.09        & 7.66         & 0.69 
 \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{We report the image retrieval performance on MMDD, PhotoChat, MMDialog, and DialogCC. The model with the best performance is indicated in \textbf{bold}, while the second best is \underline{underlined}.}
\label{main_tab:image_aug_results}

\end{table}
}

==> tables/main_tables/rating_results.tex <==
\begin{table}[t]
\centering
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{@{}lcccc@{}}
\toprule
      & \multicolumn{1}{l}{\makecell[c]{Turn\\Relevance}} & \multicolumn{1}{l}{\makecell{Rationale\\Relevance}} & \multicolumn{1}{l}{\makecell{Aligned Image \\Relevance}} & \multicolumn{1}{l}{\makecell{Image\\Consistency}} \\ \midrule
Avg.  & 3.68              & 3.41                          & 3.30                        & 3.57                         \\
$\alpha$ & 0.14                      & 0.39                       & 0.54                            & 0.50                  \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{We report the average score for each evaluation criteria and Krippendorff's $\alpha$ for inter-rater agreement.}
\label{main_tab:rating_results}

\end{table}



==> tables/supp_tables/main_dataset_statistics.tex <==
{\renewcommand{\arraystretch}{1.35}
\begin{table}[t]
\centering
\begin{adjustbox}{width=0.9\columnwidth}

\begin{tabular}{@{}lcccccc@{}}
\toprule
Dataset                          & Type       & \makecell{\# Unique \\ Dialog}      & \makecell{\# Unique \\Image}    & \makecell{Avg. \\U./D.}       & \makecell{Avg. \\I./D.} & \makecell{Avg. \\I./U.} \\ \midrule
\multirow{4}{*}{PhotoChat}       & train          & 9,890           & 8,549            & 12.69         & 1.00          & 1.00          \\
                                 & valid          & 962             & 962              & 12.69         & 1.00          & 1.00          \\
                                 & test           & 968             & 968              & 12.83         & 1.00          & 1.00          \\
                                  \cmidrule{2-7}
                                 & total          & 11,820          & 10,479           & 12.74         & 1.00          & 1.00          \\  \midrule
\multirow{4}{*}{MMDD}            & train          & 13,141          & 12,272           & 10.00         & 3.04          & 1.86          \\
                                 & valid          & 2,148           & 334              & 12.37         & 1.12          & 1.00          \\
                                 & test           & 2,390           & 682              & 12.32         & 1.12          & 1.00          \\  \cmidrule{2-7}
                                 & total          & 17,679          & 13,288           & 11.56         & 1.76          & 1.29          \\  \midrule
\multirow{4}{*}{MMDialog}        & train          & 1,059,117       & 1,509,284        & 4.56          & 2.82          & 1.36          \\
                                 & valid          & 10,000          & 23,812           & 4.54          & 2.79          & 1.36          \\
                                 & test           & 10,000          & 23,772           & 4.58          & 2.84          & 1.36          \\  \cmidrule{2-7}
                                 & total          & 1,079,117       & 1,556,868        & 4.56          & 2.82          & 1.36          \\  \midrule
\multirow{4}{*}{\textbf{DialogCC (ours)}} & train          & 68,269          & 101,877          & 8.10          & 10.25         & 6.60          \\
                                 & valid          & 7,635           & 13,842           & 8.26          & 5.78          & 3.78          \\
                                 & test           & 7,305           & 14,083           & 8.23          & 6.01          & 3.94          \\  \cmidrule{2-7}
                                 & \textbf{total} & \textbf{83,209} & \textbf{129,802} & \textbf{8.20} & \textbf{7.34} & \textbf{4.77} \\  \bottomrule                       
\end{tabular}

\end{adjustbox}
\caption{In total, DialogCC includes the
largest number of Avg. I./D. and I./U. than others. I./D.
and I./U. denote images by dialogue and images by an utterance, respectively. U./D. denotes utterances by a dialogue. More detailed statistics are in the Appendix.}
\label{main_tab:dataset_stat}

\end{table}}


